Automatic Polyp Segmentation with Multiple Kernel Dilated Convolution Network

The detection and removal of precancerous polyps through colonoscopy is the primary technique for the prevention of colorectal cancer worldwide. However, the miss rate of colorectal polyp varies significantly among the endoscopists. It is well known that a computer-aided diagnosis (CAD) system can assist endoscopists in detecting colon polyps and minimize the variation among endoscopists. In this study, we introduce a novel deep learning architecture, named MKDCNet, for automatic polyp segmentation robust to significant changes in polyp data distribution. MKDCNet is simply an encoder-decoder neural network that uses the pre-trained ResNet50 as the encoder and novel multiple kernel dilated convolution (MKDC) block that expands the field of view to learn more robust and heterogeneous representation. Extensive experiments on four publicly available polyp datasets and cell nuclei dataset show that the proposed MKDCNet outperforms the state-of-the-art methods when trained and tested on the same dataset as well when tested on unseen polyp datasets from different distributions. With rich results, we demonstrated the robustness of the proposed architecture. From an efficiency perspective, our algorithm can process at (approx 45) frames per second on RTX 3090 GPU. MKDCNet can be a strong benchmark for building real-time systems for clinical colonoscopies. The code of the proposed MKDCNet is available at https://github.com/nikhilroxtomar/MKDCNet.

==> takeout.tex <==
Bodenstedt et al.~\cite{bodenstedt2018comparative} organized "EndoVis 2015 Instrument sub-challenge" for developing new techniques and benchmarking the \ac{ML} algorithm for segmentation and tracking of the instruments on common dataset. The organizers challenged on two different tasks, (1) Segmentation, (2) Tracking. The goal of the challenge was to address the problem related to segmentation and tracking of articulated instruments in both laparoscopic and robotic surgery\footnote{\url{https://endovissub-instrument.grand-challenge.org/EndoVisSub-Instrument/}}. A comprehensive evaluation of the methods used in instrument segmentation and tracking task for minimally invasive surgery is summarized in this work~\cite{bodenstedt2018comparative}. The extensive results evaluation showed that modern deep learning was a better choice for instrument segmentation and tracking task. 

In 2017, a follow up to the previous 2015 challenge was organized called "Robotic Instrument Segmentation Sub-Challenge"\footnote{\url{https://endovissub2017-roboticinstrumentsegmentation.grand-challenge.org/}}. The challenge was part of Endoscopic vision challenge was organized at \ac{MICCAI} 2017. This challenge offered three tasks: (1) Binary segmentation task, (2) Parts based segmentation task, and (3) Instrument type segmentation task. The goal of the binary segmentation task was to separate the image into an instrument and background. Parts segmentation challenged the participants to divide the binary instrument into a shaft, wrist, and jaws. Type Segmentation challenged the participants to identify different instrument types. A detailed description of the challenge task, dataset, methodologies used by ten participating teams in different tasks, challenge design, and limitation of the challenge can be found in the challenge summary paper~\cite{allan20192017}. 


In 2019, a similar Challenge called "Robust Medical Instrument Segmentation Challenge 2019"\footnote{\url{https://robustmis2019.grand-challenge.org/}} was organized by Roß et al.~\cite{ross2020robust}. This challenge offered three tasks (1) Binary segmentation, (2) Multiple instance detection, and (3) Multiple instance segmentation. The challenge was focused on addressing two key issues in surgical instruments, \textit{Robustness} and \textit{Generalization}, and benchmark medical instrument segmentation and detection on the provided surgical instrument dataset. We participated in the binary segmentation task of the challenge. In this paper, we present our approach used for binary segmentation tasks for endoscopic instrument segmentation. 

%They used eight-fold cross-validation, where seven-fold were used for training, and one fold was used for testing. 



%Kalavakonda et al. \cite{kalavakonda2019autonomous} evaluated three deep learning architectures for binary segmentation. All the architecture was based on the encoder-decoder network. The first architecture was based on the Vanilla U-Net~\cite{ronneberger2015u}, and the other two were based on the transfer learning mechanism. 

In addition to these challenges, there are works on instrument segmentation in robot-assisted surgery~\cite{shvets2018automatic,pakhomov2019deep}, neurosurgical instrument segmentation~\cite{kalavakonda2019autonomous}, surgical instrument segmentation on minimally-invasive robot-assisted procedures~\cite{azqueta2019segmentation}, instrument tracking~\cite{laina2017concurrent}, and endoscopic instrument segmentation~\cite{isensee2020or}. 



%The learning rate for the optimizer is set to 1e-4. We prefer a lower learning rate, as it makes sure that the model parameters are updated slowly and carefully. We reduce the learning rate by a factor of 0.1 when the validation loss does not decrease in $10$ consecutive epochs, this improves our performance a lot.  We have also used early stopping to keep the model from overfitting, which is a good practice.

%We have implemented the proposed architecture using the Keras framework~\cite{chollet2015keras} with TensorFlow~\cite{abadi2016tensorflow} as backend running on the Experimental Infrastructure for Exploration of Exascale Computing (eX3), NVIDIA DGX-2 machine. As the model is having very low trainable parameters, we can set batch size up to 128, but we have chosen to use 64 in our case. We have resized the dataset from 540 x 960 pixels to 56 x 512 pixels for better utilization of the GPU and it also helps in reducing the training time. We have trained our model on 200 epochs with Nadam optimizer and dice coefficient as the loss function. The learning rate for the optimizer is set to 1e-4. We prefer a lower learning rate, as it makes sure that the model parameters are updated slowly and carefully. We reduce the learning rate by a factor of 0.1 when the validation loss does not decrease in $10$ consecutive epochs, this improves our performance a lot.  We have also used early stopping to keep the model from overfitting, which is a good practice.




New paper


% It can play a crucial role in full instrument pose estimation and improve user interaction with the robotic system.

% However, both accurate and real-time segmentation of surgical instruments in endoscopy is still a challenging issue.


% The major challenges remain in designing a lightweight deep learning model with low computational cost and high speed to be integrated with the endoscopic hardware devices to be deployed for the clinical settings.

% We propose an automated semantic segmentation architecture called NanoNet, a novel architecture for instrument segmentation in endoscopy to address this challenge.

% The main aim of the task to classify each surgical instrument's pixel into either a background class or instrument class.

% Experiments demonstrate our superior trade-off among lightweight, speed, computation, parameter use, and performance metrics.

% NanoNet achieves a dice similarity coefficient of ... and inference speed of .....which is the state-of-the-art on 2017 MICCAI EndoVis Robotic Instrument Segmentation Challenge dataset, Kvasir-SEG and Robust Medical Instrument Segmentation challenge dataset.

% Moreover, the model size is very small with only 36000 parameters. Despite of the tiny model size, the NanoNet achieves promising results. 


\ac{VCE} is a technology for capturing the video  inside the \ac{GI} tract.  It remains the first choice for screening of small bowel diseases~\cite{}. 


\acf{MIS} and robot-assisted surgery is a new field of research. In the recent years, minimally invasive surgery, computer and robotic-assisted intervention have attracted significant attention in surgical practice. \ac{MIS} is a procedure that has less or negligible cuts, less pain, and shorter hospital stay and fewer complications as compared to traditional laparoscopic surgery. \ac{MIS} gaining increasing level of trust from surgeon. Therefore, it has improved the traditional surgical procedure and help to overcome the limitations of traditional laparoscopic surgery~\cite{azqueta2020segmentation}. However, manipulation of the surgical instrument in limited restricted operating space causes problem such as limited field of view of the endoscope, reduce in surgeon's dexterity, and lacks perception of force feedback~\cite{qiu2019real}. 





Endoscopy is the technique for looking inside the body using an endoscope. 
Endoscopy (Upper \ac{GI} endoscopy) is the procedure performed by gastroenterologists who uses the endoscope to diagnose and treat the problem of the upper digestive system. Upper \ac{GI} tract includes upper part of digestive system such as esophagus, stomach and duodenum. Upper \ac{GI} endoscope can help to diagnose the conditions such as difficulty in swallowing, abdominal pain, bleeding, ulcer, and tumor. In some cases it might be necessary to take biopsy for later examination under microscope. The endoscope can be used to treat a problem such as active bleeding from ulcer. 






























































% \begin{table*}[t!]
% \footnotesize
% \def\arraystretch{1.1}
% \caption{Available instrument datasets}
% \label{tab:availabledataset}
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \toprule
% \textbf{Dataset} & \textbf{Content} & \textbf{Resolution} & \textbf{Size} &  \textbf{Task type} & \textbf{Procedure}  & \textbf{Available} \\ \midrule

% % \begin{tabular}[c]{@{}l@{}}Instrument segmentation\\ and tracking (2015)~\cite{bodenstedt2018comparative}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Rigid and robotic\\ instruments\end{tabular} & & & & \begin{tabular}[c]{@{}l@{}}Segmentation \\ and tracking\end{tabular} & Laparoscopy \\ \hline

% % \begin{tabular}[c]{@{}l@{}}Robotic Instrument \\ Segmentation (2017)~\cite{allan20192017}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Robotic surgical\\  instruments\end{tabular}  & & & & \begin{tabular}[c]{@{}l@{}}Binary segmentation,\\ part based segmentation, \\instrument segmentation\end{tabular} & 

% % \begin{tabular}[c]{@{}l@{}}Abdominal\\ porcine  \end{tabular}  \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Robotic Scene\\ Segmentation (2018)~\cite{allan20192018}\end{tabular} & \begin{tabular}[c]{@{}l@{}}Surgical instruments\\ and other  \end{tabular}& & & & \begin{tabular}[c]{@{}l@{}}Multi-instance\\  segmentation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Robotic\\ nephrectomy  \end{tabular} \\ \hline

% \begin{tabular}[c]{@{}l@{}}Robust Medical instrument\\ segmentation (2019)~\cite{ross2020robust}\end{tabular} & \begin{tabular}[c]{@{}l@{}} laparoscopic\\ instrument \end{tabular} & & & & \begin{tabular}[c]{@{}l@{}}Binary  segmentation, \\ multiple instance\\ detection,  multiple  \\ instance segmentation\end{tabular} & Laparoscopy \\ \hline

% Kvasir-Instrument~\cite{jha2020kvasir} & \begin{tabular}[c]{@{}l@{}} Diagnostic and\\ therapeutic tools\\ in endoscopic images\end{tabular} & & & & \begin{tabular}[c]{@{}l@{}}Binary segmentation\\ Detection and localization\end{tabular} & \begin{tabular}[c]{@{}l@{}}Gastroscopy\\  \& colonoscopy\end{tabular} \\ \bottomrule
% \end{tabular}
% \end{table*}



% \begin{table*}[!t]
% \centering
% \caption{Result on ISIC 2018 dataset}
% \def\arraystretch{1.2}
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \toprule
% \textbf{Method}  & \textbf{Backbone} & \textbf{Parameters} & \textbf{DSC}  & \textbf{mIoU}  & \textbf{Recall} & \textbf{Precision} & \textbf{F2-score}  & \textbf{Overall Acc} & \textbf{FPS} \\ \midrule

% NanoNet-A && 235,425  & 0.8651 & 0.8384 & 0.8517 & 0.9084  & & & \\ \hline
% NanoNet-B && 132,049 & 0.8685 & 0.8381 & 0.8629 & 0.9002   & & & \\ \hline
% NanoNet-C&& 36,561 & 0.8601 & 0.8322 & 0.8645 & 0.8831  & & & \\ 
% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}



% \begin{table}[!t]
% \caption{Result on the binary segmentation task of 2017 Robotic Instrument segmentation challenge}
% \def\arraystretch{1.2}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% Method & Parameters & Dice   & mIoU   & Recall & Precision \\ \hline
% NanoNet-A & 235,425  & 0.0000 & 0.0000 & 0.0000 & 0.0000    \\ \hline
% NanoNet-B & 132,049 & 0.0000 & 0.0000 & 0.0000 & 0.0000   \\ \hline
% NanoNet-C & 36,561 & 0.0000 & 0.0000 &0.0000 & 0.0000    \\ \hline
% \end{tabular}
% \label{tab:result}
% \end{table}

%We have evaluated NanonNet using four instrument segmentation benchmarks. The experiments demonstrates state-of-the-art speed and superior performance with all on all four datasets.
%Our main goal was to develop an efficient algorithms that requires low computational and memory requirements. 

% The dataset contains two folders i.e, Prokto and Rectum. These are two different types of procedures. These folders contain $8$ sub-folders inside them, which represents $8$ different types of surgeries. Each of these sub-folders itself contains multiple sub-folders which contains the images and their respective masks. From these $8$ sub-folders, we use $6$ sub-folders for training, $1$ sub-folder for validation and $1$ sub-folder testing. 

% We train the model using the image dataset. The sample of the training dataset and their corresponding masks can be found in the first and second column of Figure~\ref{fig:results2}. The original size of the images is 960$\times$540. We split the dataset using 80\% of dataset for training and remaining 20\% for the validation (evaluation). The training dataset was augmented and resized. We performed augmentation such as center crop, random crop, horizontal flip, vertical flip, scale augmentation, cutout, and gray-scale. The validation dataset is not augmented and is directly resized into 512$\times$256. 

%There are numerous computer vision based approaches developed for instrument segmentation~\cite{shvets2018automatic,ni2019attention}.

%Semantic segmentation is an important task in the field of computer vision. It is the task of labeling each pixel in an image with a class label that helps to distinguish different objects in an image. It can also help in improving robotics-assisted surgery by enabling the identification and precise localization of surgical instruments from the background tissue in the endoscopic images. 

% (https://arxiv.org/pdf/2006.02706v1.pdf). 
%Therefore, an accurate semantic segmentation would provide information regarding the presence of multiple instruments in the videos or images. %Many algorithms for segmentation, tracking, and detection have been proposed in the literature, however the problem of real-time semantic segmentation still remains challenge. 

%TOOD:Nikhil

% The architecture of the NanoNet follows an encoder-decoder approach as shown in figure 1. The proposed architecture uses a pre-trained MobileNetV2 model trained on the ImageNet dataset as an encoder.

%\subsubsection{Kvasir-SEG}
%\subsubsection{ISIC 2018}

% Now the concatenated feature maps pass through the modified residual block, which further increases the generalization capacity of the decoder. The output from the modified residual block is concatenated with the 3 x 3 standard convolution with the only one feature channel and a sigmoid activation. After the feature maps pass through all the four decoder block, the output of the last decoder block is fed to a 3 x 3 standard convolution which is followed by the sigmoid activation. Finally, the sigmoid activation function gives us the binary segmentation map.

% In our modified residual block, we replace the two $3\times3$ standard convolution with depth-wise separable convolution, which helps us in drastically reducing the number of parameters of the proposed architecture.

% The input image is first fed into the pre-trained MobileNetV2 encoder, after that the encoder output goes into the a modified residual block after which it is followed by a sequence decoder blocks. The decoder block uses a bilinear upsampling to increase the spatial dimension (height and width) of the input feature maps. After that, it is concatenated with the appropriate feature maps from the pre-trained encoder using the skip connection. Now the concatenated feature maps pass through the modified residual block and then the output of the modified residual block is concatenated with the 3 x 3 standard convolution with the only one feature channel. After the feature maps pass through all the four decoder block, the output of the last decoder block is fed to a 3 x 3 standard convolution which is followed by the sigmoid activation. Finally, the sigmoid activation function gives us the binary segmentation map.



% \begin{table*}[!t]
% \centering
% \caption{Result on EAD 2019 dataset}
% \def\arraystretch{1.2}
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \toprule
% \textbf{Method} & \textbf{Backbone} &\textbf{Parameters} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision}& \textbf{F2} & \textbf{Overall acc} &\textbf{FPS} \\ \hline

% UNet~\cite{ronneberger2015u} & -&- & &  & & & & \\ \hline
% DoubleUNet~\cite{jha2020doubleUNet}& &- & & & & & & & \\ \hline
% NanoNet-A & MobileNetV2 & & &  & & & & &  \\ \hline
% NanoNet-B &MobileNetV2 &  & & &  & & & & \\ \hline
% NanoNet-C &MobileNetV2 & &  &  &  & & & & \\ 
% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}



% \begin{table*}[!t]
% \centering
% \caption{Result on Endocv2020 dataset}
% \def\arraystretch{1.2}
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \toprule
% \textbf{Method} & \textbf{Backbone} &\textbf{Parameters} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision}& \textbf{F2} & \textbf{Overall acc} &\textbf{FPS} \\ \hline

% UNet~\cite{ronneberger2015u} & -&- & &  & & & & \\ \hline
% DoubleUNet~\cite{jha2020doubleUNet}& &- & & & & & & & \\ \hline
% NanoNet-A & MobileNetV2 & & &  & & & & &  \\ \hline
% NanoNet-B &MobileNetV2 &  & & &  & & & & \\ \hline
% NanoNet-C &MobileNetV2 & &  &  &  & & & & \\ 
% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}






% \begin{table*}[!t]
% \scriptsize
% \centering
% \caption{Result on 2019 CaDIS dataset}
% \footnotesize
% \begin{tabular}{l|l|l|l|l|l|l|l|l| l}
% \toprule
% \textbf{Method} & \textbf{Backbone} & \textbf{Parameters} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision} & \textbf{F2} & \textbf{Overall acc} & \textbf{FPS} \\ \midrule

% UNet~\cite{ronneberger2015u} & -&- & &  & & & & \\ %\hline
% DoubleUNet~\cite{jha2020doubleUNet}& &- & & & & & & & \\ %\hline
% NanoNet-A &MobileNetV2 &235,425 & & & & & & & \\ %\hline
% NanoNet-B &MobileNetV2 &132,049  & & & & & & & \\ %\hline
% NanoNet-C &MobileNetV2 &36,561  & & & & & & & \\


% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}




% \subsection{Ablation Study on Kvasir-Instrument}
% \subsection{Ablation Study on Robust-MIS}
% \subsection{Ablation Study for FCB}
% \subsection{Ablation Study for FCB}


%===========================================================================

% \begin{table*}[!t]
% \scriptsize
% \centering
% \caption{Result on 2019 ROBUST-MIS dataset}
% \footnotesize
% \begin{tabular}{l|l|l|l|l|l|l|l|l|l}
% \toprule
% \textbf{Method} & \textbf{Backbone} &\textbf{Parameters} & \textbf{DSC} & \textbf{mIoU} & \textbf{Recall} & \textbf{Precision}& \textbf{F2} & \textbf{Overall acc} &\textbf{FPS} \\ \hline
% UNet~\cite{ronneberger2015u} & -&- & &  & & & & \\ %\hline
% ResUNet~\cite{zhang2018road}& &- & & & & & & & \\ %\hline
% NanoNet-A &MobileNetV2 &235,425 &0.7248 &0.6701 &0.7333 &0.8806 &0.8545 &0.9898 &22.00 \\ 
% NanoNet-B &MobileNetV2 &132,049 &0.7195 &0.6621 &0.7221 &0.8856 &0.8545 &0.9898 &25.60 \\ 
% NanoNet-C &MobileNetV2 &36,561  &0.7036 &0.6402 &0.7082 &0.8394 &0.8033 &0.9864 &26.34 \\
% \bottomrule
% \end{tabular}
% \label{tab:result}
% \end{table*}



% \subsection{Evaluation Metrics}
% \label{sec:evaluationmetrics}
%For the evaluation of our model, we have chosen standard computer vision metrics such as Sørensen–dice coefficient (DSC), \ac{mIoU}, Precision, and Recall, Specificity, Accuracy and \ac{FPS}. 

% \begin{equation}{\label{eq:1}}
% \text{DSC (A,B)} = \frac{2 \times TP} {2 \times TP + FP + FN}
% \end{equation}
% %
% \begin{equation}
% \text{IoU (A,B)} = \frac{TP} {TP + FP + FN}
% \end{equation}
% %
% \begin{equation}{\label{eq:1}}
% \text{Recall}~(r) = \frac{TP} {TP + FN}
% \end{equation}
% %
% \begin{equation}{\label{eq:3}}
% \text{Precision}~(p) =\frac{TP} {TP + FP}
% \end{equation}
% %
% \begin{equation}{\label{eq:5}}
% \text{F2} = \frac{5p \times r} {4p + r}
% \end{equation}
% %
% \begin{equation}{\label{eq:6}}
% \text{Overall accuracy}~(Acc.) ={\frac{TP + TN} {TN + TN + FP + FP}} 
% \end{equation}
% %
% \begin{equation}{\label{eq:7}}
% \text {Frame Per Second}~(FPS) = {\frac{1} {sec /frame}}
% \end{equation}

% In the above equations, \textit{TP}, \textit{FP}, \textit{TN}, \textit{FN} represents true positives, false positives, true negatives, and false negatives, respectively, for the classification outputs. Based on these metrics, we will evaluate and compare the performance of our method. 




% \subsubsection{Robust-MIS Dataset}
% The first dataset used in the study is from the Robust Medical Instrument Segmentation (ROBUST-MIS)\footnote{\scriptsize \url{https://robustmis2019.grand-challenge.org}}. Heidelberg Colorectal (HeiCo) data set~\cite{maier2020heidelberg} includes a total of $5983$ images with their respective manually annotated masks. These training images are obtained from $16$ different surgeries with the two different types of procedures (Prokto and Rectum, $8$ surgeries each). The prokto consists of $2943$ images, and the rectum contains $3040$ images. The challenge also offers a video dataset. However, we have not used a video dataset for our experimental setup. 

% \subsubsection{Endovis Robotic Instrument segmentation Challenge dataset}
% The dataset is taken from the "Robotic Instrument Segmentation challenge" held at the 2017 MICCAI Endovis Challenge. The video frames are acquired from a da Vinci Xi robot. These images are from various porcine procedures. The dataset consists of 3000 images, out of which 1800 images were used for training, and 1200 images were used for testing. The images have a resolution of $1280\times1024$. There are seven types of surgical instruments in Endovis 2017. More details about the challenge and challenge dataset can be found from here \footnote{\scriptsize {\url{https://endovissub2017-roboticinstrumentsegmentation.grand-challenge.org/}}


%The paper is organized as follows. Section \ref{sec:relatedwork} describes the related work on instrument segmentation and highlights the need for real-time segmentation. Section \ref{sec:methods} describes the NanoNet architectures used in our study. Section \ref{sec:materials used} describes the material used to validate the proposed method. Section \ref{sec:results} describes the results. Section \ref{sec:Discussion} describes the discussion. Section \ref{sec:conclusion} describes the conclusion and highlights the future work. 


%This is an important contribution for vision-based minimal invasive surgery and can be useful for clinical trails.

%Moreover, we will investigate ways to optimize the network for achieving higher performance with the same number of parameters. We will work on detection and localization of the surgical instrument in near future. 



%Real-time segmentation of the endoscopy is a challenging problem. An automated pixel-wise segmentation of endoscopic images can reduce the risk for miss-detection. These applications can reduce the doctors' burden, improve the overall performance and clinical workflow. The semantic segmentation of medical images (colonosopic images) are challenging as compared to the segmentation of the natural images. It is challenging due to variation in lighting, shadows, the overlap between the instrument, reflection, occlusions from blood, fogging, or interference from the surgeon in the frame~\cite{bouget2017vision}. These challenges presence makes it difficult to distinguish between the polyp and background tissue. 

%\ac{MIS} gaining increasing level of trust from surgeon. Therefore, it has improved the traditional surgical procedure and help to overcome the limitations of traditional laparoscopic surgery~\cite{azqueta2020segmentation}.












%%%%%%new%%%%%%%%%%%%%%%%%%%%%%


%A lightweight model is preferred to be used in clinical settings. Moreover, the inference time of the Nanonet is real-time, and the model does not require any sort of initialization or post-processing, or temporal regularization, which can be considered as the strength of the work. 

%In the future, we plan to design an encoder from scratch, which can be even lighter than pre-trained MobilNetV2. We also plan to work with the medical experts to understand the images and procedure in-depth to group the segment and distinguish between semantically meaningful information. 
% In this paper, we proposed a novel lightweight architecture, NanoNet, designed for endoscopic image segmentation. The improved performance of the NanoNet is due to the use of a lightweight pre-trained MobileNetV2 model and modified residual block. The depthwise separable convolution is the main building block of the network because of which our model can achieve high performance with fewer trainable parameters. The experimental result on recent segmentation benchmarks on five endoscopy datasets demonstrates state-of-the-art speed and performance.  A lightweight model is preferred to be used in clinical settings. Moreover, the inference time of the Nanonet is real-time, and the model does not require any sort of initialization or post-processing, or temporal regularization, which can be considered as the strength of the work. In the future, we plan to design an encoder from scratch, which can be even lighter than pre-trained MobilNetV2. We also plan to work with the medical experts to understand the images and procedure in-depth to group the segment and distinguish between semantically meaningful information. 


%Chaurasia et al.~\cite{paszke2016enet} proposed efficient neural network (EDNet), that was especially designed for high accuracy and fast inference. The model was 18 times faster and requires less parameter providing similar accuracy on the CamVid, Cityscapes and SUN datasets. Garcia-Peraza-Herrera et al.~\cite{garcia2017toolnet} proposed two architectures, TOOLNetMS and ToolNetH that were trained end-to-end for real-time semantic segmentation of surgical tools. Yu et al.~\cite{yu2018bisenet} proposed bilateral segmentation network (BiSeNet) for improving the speed and accuracy for the real-time semantic segmentation. The model consists of spatial path and context path for preserving spatial information from the original images. This network makes the right balance between accuracy and speed on the CamVid, Cityscapes and SUN datasets. 


% \subsection{Dataset}
% \begin{figure}
%     \centering
%      \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/1.jpg}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/1_mask.png}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/2.jpg}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/2_masks.png} \\
%         \vspace{1mm}
%       \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/3.jpg}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/3_mask.png}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/4.jpg}
%         \includegraphics[width=1.9cm, height=1.9cm]{figures/data_sample/4_mask.png}
%     \caption{Example dataset from Kvasir-Instrument}
%     \label{fig:kvasir-instrument}
% \end{figure}


% \subsection{Generalisability} 
% Generalization is the ability of the model to perform well on other institute datasets  or interventions.  To promote the generalization, we have tested our best methods trained on Kvasir-SEG with the CVC-ClinicDB dataset. The performance of the best detection, localisation, and segmentation methods have shown that the methods have good accuracy and generalization capabilities. However, the model's performance was not as good as they perform while trained and tested on the same dataset. This can be evidence by the quantitative and qualitative results (see Table~\ref{tab:resultEndotect2020,tab:resultMedico2020} and Figure~\ref{qualitativeresultsa}). This may be because two different images are captured using different endoscopic devices, making it difficult to generalize.


% \subsection{Kvasir-Instrument dataset}
% Kvasir-Instrument~\cite{jha2020kvasirInstrument} is publicly available datasets and consist of 590 frames from \ac{GI} endoscopy. These images are from various therapeutic or surgical procedures. These datasets are collected using standard endoscopic equipment from Olympus and Pentax. The dataset consists of original images, ground truth, and bounding box information. %The example of the dataset is shown in the Figure~\ref{fig:kvasir-instrument}. 


%We have curated a dataset for the generalizability test or domain adaptation test. Therefore, we train the model on the colonoscopy dataset and test it against the \ac{VCE} dataset.


% We only have the training dataset provided by the challenge organizers, so we use that dataset for training, validation and testing purpose. The dataset is obtained from two different procedures (Prokto and Rectum), each contain data for $8$ surgeries each. Out of these $8$ surgeries, we have used $6$ surgeries for training, $1$ for validation and $1$ for testing purpose. The original resolution of the images is $540 \times 960$. For our convenience, we resized all the images to $256\times512$.


%Despite the small model size, the NanoNet achieves competitive results, which is the major strength of the work. 

%Deep learning in gastrointestinal endoscopy has tremendous potential to improve clinical performance and assessment of patients. The semantic segmentation of an image can provide critical information during medical examinations, which can play a crucial role in patient safety. However, accurate and real-time segmentation of endoscopic images is still a challenging problem. The significant challenges remain in designing a lightweight deep learning model with low computational cost and high speed to be integrated with the endoscopic hardware devices to be deployed for the clinical settings. To improve the eminent problems in diagnosis endoscopy systems, we propose a novel automated architecture, NanoNet, for segmenting endoscopic images. Experimental results demonstrate that NanoNet achieves promising results for wireless capsule endoscopy, colonoscopy, tools, and surgical instrument images. Experiments show our superior trade-off among lightweight, speed, computation, parameter use, and performance metrics. Moreover, the model size is tiny, with only 36000 parameters. Despite the small model size, the NanoNet achieves promising results, which is the major strength of the work. 

%Convolutional neural networks can play a crucial role in assisting clinicians. There has been a significant progress in the area of medical image analysis, especially with the development of medical diagnosis support systems for assisting clinicians. Such systems can offer better medical diagnoses, which can positively impact the patient's health. However, the significant challenges remain within the availability of high-quality, diverse labeled medical datasets for experimentation to develop such clinically relevant systems.


%Upper \ac{GI} is consists of the esophagus, stomach, and duodenum. Endoscopy (Upper \ac{GI} endoscopy) is the procedure where gastroenterologists observe an internal organ inside the body using an endoscope. Upper \ac{GI}  endoscope helps diagnose the conditions such as bleeding, ulcer, tumor, abdominal pain, and trouble in swallowing. A biopsy is taken for further investigation in cases where gastroenterologists encounter suspicious tissue. Endoscopy is also useful for treatment (for example, active bleeding for ulcers).  

%In recent years, \ac{MIS}, computer and robotic-assisted intervention have attracted significant attention in surgical practice. It is a procedure that has fewer or minor cuts, less pain, and requires a shorter hospital stay and fewer complications as compared to traditional laparoscopic surgery. However, manipulation of the surgical instrument is limited, restricted operating space causes a problem such as limited field of view of the endoscope, reduction in surgeon's dexterity, and lacks the perception of force feedback~\cite{qiu2019real}.  

%Upper \ac{GI} consists of the esophagus, stomach, and duodenum. The lower \ac{GI} consists of the large intestine and anus. 




, each beginning with a bilinear upsampling followed by the concatenation of the feature maps from the MKDC block. Next, two residual blocks are used to learn the required semantic features that would help the network to generate a better segmentation mask. 

The multiscale feature fusion (MSFF) block takes the output of three decoder blocks and combines them to produce a more refined output.








%--------------------------------------------------------------------------------------------------------------------------------------------------


% \midrule

% \multicolumn{8}{@{}l}{\textbf{Train Dataset: Kvasir-SEG\cite{jha2020kvasir}, Test Data: Unseen CVC-ClinicDB~\cite{bernal2015wm}}}                   \\ \hline
% U-Net~\cite{ronneberger2015u}	&0.6336	&0.5433	&0.6982	&0.7891	&0.9484	&0.6563	&166.05\\
% ResU-Net~\cite{zhang2018road}	&0.5970	&0.4967	&0.6210	&0.8005	&0.9465	&0.5991	&\textbf{195.38}\\
% U-Net++~\cite{zhou2018unet++}	&0.6350	&0.5475	&0.6933	&0.7967	&0.9504	&0.6556	&127.80\\
% ResU-Net++~\cite{jha2019resunet++}	&0.4642	&0.3585	&0.5880	&0.5770	&0.9159	&0.5084	&57.96\\
% % ColonSegNet~\cite{jha2021real}	&0.6126	&0.5090	&0.6564	&0.7521	&0.9440	&0.6246	&132.32\\
% HarDNet-MSEG~\cite{huang2021hardnet}	&0.6960	&0.6058 &0.7173	&0.8528	&0.9592	&0.7010	&42.38\\
% DeepLabV3+ (ResNet50)~\cite{chen2018encoder}	&0.8142	&0.7388	&0.8331	&0.8735	&\textbf{0.9717}	&0.8198	&103.17\\
% DDANet\cite{tomar2021ddanet}	&0.5234	&0.4183	&0.6502	&0.5935	&0.9275	&0.5718	&91.32\\
% \textbf{DeepSegNet (Ours)}	&\textbf{0.8243}	&\textbf{0.7466}	&\textbf{0.8494}	&\textbf{0.8637	}&0.9709	&\textbf{0.8325}	&46.71\\
% \midrule

% \multicolumn{8}{@{}l}{\textbf{Train Dataset: Kvasir-SEG\cite{jha2020kvasir}, Test Data: Unseen BKAI-IGH~\cite{lan2021neounet}}}  
%  \\ \hline
% U-Net~\cite{ronneberger2015u} &0.6347	&0.5686	&0.6986	&0.7882	&0.9753	&0.6591	&162.60 \\
% ResU-Net~\cite{zhang2018road} &0.5836	&0.4931	&0.6716	&0.6549	&0.9671	&0.6177	&\textbf{199.02} \\
% U-Net++~\cite{zhou2018unet++} &0.6269	&0.5592	&0.6900	&0.7968	&0.9741	&0.6493	&128.59 \\
% ResU-Net++~\cite{jha2019resunet++} &0.4166	&0.3204	&0.6979	&0.3922	&0.9061	&0.5019	&57.22 \\
% % ColonSegNet~\cite{jha2021real} &0.5765	&0.4910	&0.7191	&0.6644	&0.9503	&0.6225	&130.21 \\
% HarDNet-MSEG~\cite{huang2021hardnet} &0.6502	&0.5711	&0.7420	&0.7469	&0.9713	&0.6830	&42.44 \\
% DeepLabV3+ (ResNet50)~\cite{chen2018encoder} &0.7286	&0.6589	&0.7919	&0.8123	&\textbf{0.9787}	&0.7493	&103.25 \\
% DDANet\cite{tomar2021ddanet} &0.5006	&0.4115	&0.6612	&0.4825	&0.9507	&0.5592	&91.73 \\
% \textbf{DeepSegNet (Ours)} &\textbf{0.7483}	&\textbf{0.6782}	&\textbf{0.8087}	&\textbf{0.8155}	&0.9756	&\textbf{0.7651}	&42.741 \\
% \midrule

% \multicolumn{8}{@{}l}{\textbf{Train Dataset: BKAI-IGH\cite{lan2021neounet}, Test Data: CVC-ClinicDB~\cite{bernal2015wm}}}                   \\ \hline
% U-Net\cite{ronneberger2015u}&	0.6588	&0.5715	&0.6518	&0.8722	&0.9528	&0.6487	&\textbf{162.02}\\
% ResU-Net\cite{zhang2018road}	&0.4670	&0.3769	&0.4158	&0.8354	&0.9351	&0.4310	&124.55\\
% U-Net++\cite{zhou2018unet++}	&0.6227	&0.5360	&0.5941	&0.8797	&0.9499	&0.6009	&125.83\\
% ResU-Net++\cite{jha2019resunet++}	&0.6190	&0.5128	&0.6319	&0.7469	&0.9467	&0.6158	&58.7\\
% ColonSegNet\cite{jha2021real}	&0.5666	&0.5666	&0.5963	&0.7386	&0.9304	&0.5664	&135.29\\
% HarDNet-MSEG~\cite{huang2021hardnet}	&0.6493	&0.5516	&0.6325	&0.8298	&0.9527	&0.6340	&41.145\\
% DeepLabV3+ (ResNet50)~\cite{chen2018encoder}	&\textbf{0.7583}	&\textbf{0.6816}	&\textbf{0.7536}	&\textbf{0.9093}	&\textbf{0.9652}	&\textbf{0.7521}	&101.44\\
% DDANet\cite{tomar2021ddanet}	&0.5873	&0.4770	&0.6176	&0.7118	&0.9424	&0.5918	&89.183\\
% \textbf{DeepSegNet (Ours)}	&0.7393	&0.6635 &0.7241	&0.9059	&0.9627	&0.7257	&47.96\\

























